Scaling Safe Multi-Agent Control for Signal Temporal Logic Specifications

Existing methods for safe multi-agent control using logic specifications like Signal Temporal Logic (STL) often face scalability issues. This is because they rely either on single-agent perspectives or on Mixed Integer Linear Programming (MILP)-based planners, which are complex to optimize. These methods have proven to be computationally expensive and inefficient when dealing with a large number of agents. To address these limitations, we present a new scalable approach to multi-agent control in this setting. Our method treats the relationships between agents using a graph structure rather than in terms of a single-agent perspective. Moreover, it combines a multi-agent collision avoidance controller with a Graph Neural Network (GNN) based planner, models the system in a decentralized fashion, and trains on STL-based objectives to generate safe and efficient plans for multiple agents, thereby optimizing the satisfaction of complex temporal specifications while also facilitating multi-agent collision avoidance. Our experiments show that our approach significantly outperforms existing methods that use a state-of-the-art MILP-based planner in terms of scalability and performance. The project website is https://jeappen.com/mastl-gcbf-website/ and the code is at https://github.com/jeappen/mastl-gcbf .

==> sections/5_approach.tex <==
\section{Approach}

\subsection{Differentiable Signal Temporal Logic}
Signal Temporal Logic (STL) provides a robustness metric for a given trajectory that quantifies the level of satisfaction of a specification $\phi$ defined using the STL language.
Prior work \citep{xiong2023colearning}  has used this feature to refine a planner's waypoints for use by a given Low-level controller.
Motivated by their success, we define a planner that attempts to maximize the MA-STL robustness score and provides separate timed waypoints. 

\subsection{GNNs for Planning in Multi-Agent Systems}
\label{sec:gnn-plan}
Graphical models can be useful to scale collision avoidance in multi-agent systems \citep{yu2022learning} by modeling the system in a decentralized manner. 
For an egocentric graph observation $G_i = \langle V, E \rangle$, on an agent $i$, a planner $P_G$ yields $P_G(G_i, \phi) = \Delta p_i$ 
being the deviation from the current goal and we can repeat this on the next state  for $K$ waypoints $\langle p_i^1, \ldots p_i^K \rangle$. 

\iffalse

These waypoints form a Piece-wise Linear (PWL) plan which the agents must follow.


Since MA-STL specifications require timed waypoints to satisfy the time constraints of the STL specification, we associate a time $t_i^j$ for $1\leq j \leq K$ with each waypoint as well.
The planner thus outputs these two components as the timed waypoint based on the current observation.
This time must increase monotonically to be consistent and these waypoints need to satisfy the collision-avoidance property as well.

For monoticity of the time we use the neural network to predict a non-negative increment on the time of the previous waypoint $\Delta t_i^j = t_i^j - t_i^{j-1} > 0$ for $j>=1$ and use this to specify the time for each waypoint.
Non-negative activation functions such as ReLU nodes can be used to enforce this constraint.

For a PWL plan to avoid collisions between agents when following an $\epsilon$-robust controller, these timed waypoints either need to be time-disjoint or space-disjoint \citep{Sun2022}. 
We incorporate a loss capturing this objective $\mathcal{L}_{coll}$. 


To begin, let's examine how to represent the specification that two time-stamped line segments are at least $\epsilon$ apart, serving as the foundation for encoding the inter-agent collision avoidance requirement. We consider two time-stamped line segments, $\mathtt{SEG}_1$ and $\mathtt{SEG}_2$, with endpoints$(t_{11}, p_{11})$ and $(t_{12}, p_{12})$ , and $(t_{21}, p_{21})$ and $(t_{22}, p_{22})$ respectively. We define the function $\safe()$, mapping them to an LCF (Logical Constraint Formula) as follows:

\begin{align*}
	\safe_{\mathtt{SEG}_1, \mathtt{SEG}_2, \epsilon} := & \left([t_{11}, t_{12}] \cap [t_{21}, t_{22}] = \varnothing\right) \ \vee \\
	& \Bigg(\left|\frac{p_{11}+p_{12}}{2} - \frac{p_{21}+p_{22}}{2}\right|_2 \geq \quad \ \left|\frac{p_{11}-p_{12}}{2}\right|_2 + \left|\frac{p_{21}-p_{22}}{2}\right|_2 + \epsilon \sqrt{d}\Bigg),
\end{align*}

where d represents the workspace's dimensionality. Essentially, if the above LCF holds, one of the following two conditions is true: either the segments are disjoint in the time dimension, or in the spatial dimension. If the distance between their centers exceeds the sum of their half-lengths plus a margin $\epsilon$, this indicates spatial disjointness.

Next, the specification ensuring that all agents avoid collisions with one another can be encoded as:

\begin{equation*}
	z_{\texttt{inter}} = \bigwedge_{\substack{i, j = 1\ i \neq j}}^{N} ~ \bigwedge_{\substack{k=1,\dots,K_i\ l=1,\dots,K_j}} \safe\left(S_i^{(k)}, S_j^{(l)}, 2\epsilon + s_i + s_j\right),
\end{equation*}

This equation, once again an LCF, incorporates the decision variables $\bigcup_{i=1}^{N}\bigcup_{k=0}^{K_i}{t^k_{i}, p^k_{i}}$. Recall that $s_i$ represents the size of agent i.
To translate this LCF to a loss differentiable loss function for the neural planner, we replace $\land$ with $\min$ and $\lor$ with $\max$ as mentioned in Sec. \ref{bg-stl}.

$$\mathcal{L}_{coll} = \min_{\substack{i, j = 1\ i \neq j}}^{N} ~ \min_{\substack{k=1,\dots,K_i\ l=1,\dots,K_j}} \safe\left(S_i^{(k)}, S_j^{(l)}, 2\epsilon + s_i + s_j\right),$$

\fi

Thus the loss for the planner is $\mathcal{L} = \mathcal{L}_{coll} + \mathcal{L_\phi}$ where
$\mathcal{L_\phi} = -\sum_{i\in \mathcal{N}} \rho(\tau_i) $. 
We sample trajectories $\tau$ and calculate the robustness score for each agent $i$ using $\rho_i (\tau_i)$ and maximize this w.r.t. planner parameters $\omega_p$.
By iteratively carrying out this optimization using gradient descent on sampled trajectories, we can perform other optimizations in between iterations to 
reduce the need of planning for collision-avoidance as shown below in Section \ref{sec:app-cam}.

 
\subsection{Collision Avoidance in MA Systems}

\label{sec:app-cam}

We use the end-to-end differentiable nature of learning-based collision avoidance schemes to ensure the safety of the system 
while updating the controller to satisfy the specification as well. Control Admissibility Models (CAMs) \citep{yu2022learning} 
ensure safety of the MA system by restricting the action space to safe actions dependent on the behavior of other agents.
They provide a egocentric based view of the agent and its nearby agents upon which the CAM is trained on a small group of agents (say $N=3$ agents).
 The CAM is then deployed on a larger number agents which is then used to limit actions based on aggregation of the admissibility models
 on multiple subsets of the agents. 

This has been shown to be scalable in terms of the number of agents and fits our requirement of a differentiable approach to collision avoidance.
Thus we choose CAMs as our primary safety mechanism during execution of MA system and incorporate our planner to provide a goal for use by the 
controller.

Since the controllers are learned iteratively, we also sample and update the $\epsilon$ term used in our loss 
function denoting the tracking error of these controllers.
%\subsection{Signal Temporal Logic for Multi-agent Systems}
%\label{ap-stl}


\subsection{Planning for MA-STL}

As highlighted in Sec. \ref{bg-stl}, MA-STL can be thought of as \textit{independent} single-agent STL specifications on the agents albeit with an additional 
constraint on avoiding collisions between the agents. While collision avoidance during planning time is expensive (Sec. 
\ref{sec:ps-stl}), we can attempt to plan for the objectives for a subset of the agents and use this plan with a safety
scheme during run-time.

However this may detract from the overall objective, thus we update the planner iteratively by sampling the environment as detailed in Sec. \ref{sec:gnn-plan}
with the STL robustness score. Thus we "co-learn" the safety and objective behavior which is a recurrent theme in recent work \citep{xiong2023colearning, Xiong2022}
related to the safety of controllers in complex systems.

If this plan with timed waypoints is capable of being satisfied in a $\epsilon$-robust manner for
\textit{all} subsets of agents we planned for, then the overall MA-STL specification $\Psi$ is satisfied.
One should note, this would not be the case if we had defined arbitrary STL specifications in the joint space of agents
involving global coordination or synchronization of objectives (i.e. global predicate functions \citep{Eappen2022}).
In that situation, an $\epsilon$-robust realization of a plan on different subsets of the agents would not directly translate to 
the specification being satisfied on the entire set of agents.

%\section{ALGORITHM}
%There are two variants of our MARL algorithm:
%\subsection{Run-time Communication needed}
%\begin{enumerate}
%	\item Agents need to use sensors to communicate with other agents and determine the RoA they decide to use during run-time
%	
%\end{enumerate}
%
%\begin{itemize}
%	\item Pros: More robust, synchronized with run-time data,
%	\item Cons: Communication may be expensive and delayed
%\end{itemize}
%\subsection{Run-time Communication minimized}
%\begin{enumerate}
%	\item Agents use knowledge of the expected plan of the other agents (along with the way-point times).
%	\item Assumptions are made on the controller and RoA shield use during run-time which are then used to predict position of other agents at a given time.
%	
%\end{enumerate}
%
%\begin{itemize}
%	\item Pros: Minimize communication needed between agents
%	\item Cons: Makes assumptions on controller capabilities and agent position ignoring real-time disturbances. Agents may deviate from given plans significantly. May be expensive to handle conflicts during plan-time.
%\end{itemize}

==> sections/A4_hardness_of_mastl.tex <==
\section{Hardness of MA-STL specifications}

We also performed an ablation study (Table \ref{tab:single-safety-performance}, \ref{tab:dubins-safety-performance}, \ref{tab:double-safety-performance}) to emphasize the challenge of satisfying these individual temporal objectives while ensuring global constraints such as safety (collision avoidance).
%\SJ{What does safety mean here - collision avoidance or goal satisfaction}, 
%we perform a related ablation study (Table \ref{tab:safety-performance}) showcasing how our approach balances liveness (or performance) and safety. 
For each specification, we use the MILP planner with \gcbfp~controller and consider the case of an algorithm prioritizing safety above all else while sacrificing objective satisfaction (i.e. by attempting to remain stationary rather than risking collisions when a collision is detected 1 step ahead).
This method (marked `Prioritize Safety') uses environment dynamics and global agent communication to perform this one step lookahead. 
Notably this is not guaranteed to be safe due to agent input limits and is unrealistic since it is not decentralized.
We compare this to an algorithm with the MILP planner that can satisfy the temporal specifications nearly always yet allows collisions between agents by simply following the nominal controller (PID with no collision avoidance maneuvering \citep{zhang_gcbf_2024}) marked `Prioritize Objective'.

From the results in Table \ref{tab:dubins-spec-v-n-results} we can see the non-linear nature of the DubinsCar environment, and input limits, hinders a near 100\% safety rate in the `Prioritize Safety' variant unlike in the other linear environments (Tables \ref{tab:single-safety-performance}, \ref{tab:double-safety-performance}).
Additionally based on the results we can see in the more complex environments (DubinsCar, DoubleIntegrator) the overly conservative approach of `Prioritize Safety' affects finish rates negatively in the $N=32$ case (even with the expensive global communication).
These results highlight the need for planning informed of collision avoidance procedures.

\begin{table*}[t!]
	\centering
	\scalebox{0.7}{
		\begin{tabular}{l|l|cccc|cccc}
			\toprule
			%	\multicolumn{3}{c|}{Planner} & \multicolumn{6}{c|}{GNN-ODE (Ours)} & \multicolumn{6}{c|}{ODE} & \multicolumn{6}{c}{STLPY} \\//
			\multicolumn{2}{c|}{Planner} & \multicolumn{4}{c|}{Prioritize Objective} & \multicolumn{4}{c}{Prioritize Safety} \\
			\midrule
			Spec & N & Finish Rate $\uparrow$ & Safety Rate $\uparrow$ & Success Rate $\uparrow$ & TtR $\downarrow$ & Finish Rate $\uparrow$ & Safety Rate $\uparrow$ & Success Rate $\uparrow$ & TtR $\downarrow$ \\
			%	Spec & N &  &  &  &  &  &  &  &  \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Branch}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{F6A385} 20.00 & \cellcolor[HTML]{F6A385} 20.00 & \cellcolor[HTML]{3B4CC0} 233.25 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{4B64D5} 256.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{C73635} 2.50 & \cellcolor[HTML]{C73635} 2.50 & \cellcolor[HTML]{3D50C3} 236.12 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{5F7FE8} 290.50 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3C4EC2} 234.88 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{465ECF} 95.00 & \cellcolor[HTML]{465ECF} 95.00 & \cellcolor[HTML]{7A9DF8} 342.44 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Cover}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{D44E41} 5.00 & \cellcolor[HTML]{D44E41} 5.00 & \cellcolor[HTML]{6A8BEF} 309.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{7EA1FA} 350.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{6A8BEF} 310.25 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{90B2FE} 386.00 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{6A8BEF} 310.12 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B7CFF9} 471.50 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Loop}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{F0CDBB} 654.75 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{F7AF91} 751.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{F0CDBB} 654.75 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{ED8366} 855.38 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{EFCEBD} 653.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 1053.81 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Sequence}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{A1C0FF} 419.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B6CEFA} 468.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{A2C1FF} 422.75 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{D8DCE2} 563.75 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{A1C0FF} 421.62 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3D50C3} 98.75 & \cellcolor[HTML]{3D50C3} 98.75 & \cellcolor[HTML]{F7B093} 748.12 \\
		\end{tabular}
	}
	\caption{Depicting the balance between performance and safety with regards to STL specification complexity for the SingleIntegrator Environment at various scales.}
	\label{tab:single-safety-performance}
\end{table*}


\begin{table*}[t!]
	\centering
	\scalebox{0.7}{
		\begin{tabular}{l|l|cccc|cccc}
			\toprule
			%	\multicolumn{3}{c|}{Planner} & \multicolumn{6}{c|}{GNN-ODE (Ours)} & \multicolumn{6}{c|}{ODE} & \multicolumn{6}{c}{STLPY} \\//
			\multicolumn{2}{c|}{Planner} & \multicolumn{4}{c|}{Prioritize Objective} & \multicolumn{4}{c}{Prioritize Safety} \\
			\midrule
			Spec & N & Finish Rate $\uparrow$ & Safety Rate $\uparrow$ & Success Rate $\uparrow$ & TtR $\downarrow$ & Finish Rate $\uparrow$ & Safety Rate $\uparrow$ & Success Rate $\uparrow$ & TtR $\downarrow$ \\
			%	Spec & N &  &  &  &  &  &  &  &  \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Branch}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{F7B599} 25.00 & \cellcolor[HTML]{F7B599} 25.00 & \cellcolor[HTML]{3B4CC0} 330.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{92B4FE} 370.50 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{CB3E38} 3.75 & \cellcolor[HTML]{CB3E38} 3.75 & \cellcolor[HTML]{4961D2} 335.12 & \cellcolor[HTML]{485FD1} 98.00 & \cellcolor[HTML]{4C66D6} 92.50 & \cellcolor[HTML]{4C66D6} 92.50 & \cellcolor[HTML]{EDD1C2} 434.55 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.62 & \cellcolor[HTML]{B40426} 0.62 & \cellcolor[HTML]{4055C8} 332.25 & \cellcolor[HTML]{B40426} 65.00 & \cellcolor[HTML]{B7CFF9} 56.25 & \cellcolor[HTML]{CFDAEA} 47.50 & \cellcolor[HTML]{B40426} 540.42 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Cover}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{D44E41} 5.00 & \cellcolor[HTML]{D44E41} 5.00 & \cellcolor[HTML]{3C4EC2} 447.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{4358CB} 95.00 & \cellcolor[HTML]{4358CB} 95.00 & \cellcolor[HTML]{7EA1FA} 483.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3C4EC2} 447.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 98.75 & \cellcolor[HTML]{3B4CC0} 98.75 & \cellcolor[HTML]{F4C6AF} 588.00 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3B4CC0} 447.00 & \cellcolor[HTML]{B40426} 80.00 & \cellcolor[HTML]{82A6FB} 72.50 & \cellcolor[HTML]{A5C3FE} 61.25 & \cellcolor[HTML]{B40426} 704.72 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Loop}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3B4CC0} 1006.00 & \cellcolor[HTML]{7A9DF8} 95.00 & \cellcolor[HTML]{3B4CC0} 90.00 & \cellcolor[HTML]{3B4CC0} 85.00 & \cellcolor[HTML]{6E90F2} 1087.79 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3E51C5} 1009.12 & \cellcolor[HTML]{516DDB} 98.00 & \cellcolor[HTML]{5D7CE6} 77.50 & \cellcolor[HTML]{5470DE} 76.25 & \cellcolor[HTML]{F4987A} 1568.79 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3B4CC0} 1006.31 & \cellcolor[HTML]{B40426} 79.00 & \cellcolor[HTML]{B3CDFB} 51.25 & \cellcolor[HTML]{C1D4F4} 44.38 & \cellcolor[HTML]{B40426} 1810.24 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Sequence}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3B4CC0} 582.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{A6C4FE} 682.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{445ACC} 588.50 & \cellcolor[HTML]{81A4FB} 95.00 & \cellcolor[HTML]{4358CB} 96.25 & \cellcolor[HTML]{4961D2} 93.75 & \cellcolor[HTML]{F5C1A9} 814.29 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{4358CB} 587.12 & \cellcolor[HTML]{B40426} 81.00 & \cellcolor[HTML]{88ABFD} 71.25 & \cellcolor[HTML]{A3C2FE} 62.50 & \cellcolor[HTML]{B40426} 992.41 \\
		\end{tabular}
	}
	\caption{Depicting the balance between performance and safety with regards to STL specification complexity for the DubinsCar Environment at various scales.}
	\label{tab:dubins-safety-performance}
\end{table*}


\begin{table*}[t!]
	\centering
	\scalebox{0.7}{
		\begin{tabular}{l|l|cccc|cccc}
			\toprule
			%	\multicolumn{3}{c|}{Planner} & \multicolumn{6}{c|}{GNN-ODE (Ours)} & \multicolumn{6}{c|}{ODE} & \multicolumn{6}{c}{STLPY} \\//
			\multicolumn{2}{c|}{Planner} & \multicolumn{4}{c|}{Prioritize Objective} & \multicolumn{4}{c}{Prioritize Safety} \\
			\midrule
			Spec & N & Finish Rate $\uparrow$ & Safety Rate $\uparrow$ & Success Rate $\uparrow$ & TtR $\downarrow$ & Finish Rate $\uparrow$ & Safety Rate $\uparrow$ & Success Rate $\uparrow$ & TtR $\downarrow$ \\
			%	Spec & N &  &  &  &  &  &  &  &  \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Branch}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{DC5D4A} 7.50 & \cellcolor[HTML]{DC5D4A} 7.50 & \cellcolor[HTML]{3B4CC0} 316.25 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{D5DBE5} 427.50 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{CB3E38} 3.75 & \cellcolor[HTML]{CB3E38} 3.75 & \cellcolor[HTML]{465ECF} 321.38 & \cellcolor[HTML]{8FB1FE} 91.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{506BDA} 91.25 & \cellcolor[HTML]{E57058} 547.60 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.62 & \cellcolor[HTML]{B40426} 0.62 & \cellcolor[HTML]{4257C9} 319.06 & \cellcolor[HTML]{B40426} 71.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{89ACFD} 71.25 & \cellcolor[HTML]{B40426} 602.46 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Cover}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{DE614D} 7.50 & \cellcolor[HTML]{DE614D} 7.50 & \cellcolor[HTML]{3B4CC0} 404.50 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{A5C3FE} 520.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3B4CC0} 404.75 & \cellcolor[HTML]{5E7DE7} 98.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{4055C8} 97.50 & \cellcolor[HTML]{F39577} 745.25 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{BA162B} 0.62 & \cellcolor[HTML]{BA162B} 0.62 & \cellcolor[HTML]{3B4CC0} 404.50 & \cellcolor[HTML]{B40426} 86.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{5D7CE6} 86.25 & \cellcolor[HTML]{B40426} 885.43 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Loop}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3B4CC0} 812.25 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{93B5FE} 1207.25 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3B4CC0} 812.88 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{EAD4C8} 1800.38 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3C4EC2} 814.44 & \cellcolor[HTML]{B40426} 95.00 & \cellcolor[HTML]{3D50C3} 98.75 & \cellcolor[HTML]{465ECF} 95.00 & \cellcolor[HTML]{B40426} 2861.72 \\
			\hline\multirow[t]{3}{*}[-1em]{\STAB{\rotatebox[origin=c]{90}{\footnotesize Sequence}}} & 8 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{C73635} 2.50 & \cellcolor[HTML]{C73635} 2.50 & \cellcolor[HTML]{3B4CC0} 535.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{E5D8D1} 770.00 \\
			& 16 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{BE242E} 1.25 & \cellcolor[HTML]{BE242E} 1.25 & \cellcolor[HTML]{3E51C5} 537.75 & \cellcolor[HTML]{7597F6} 86.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{5D7CE6} 86.25 & \cellcolor[HTML]{CA3B37} 1009.40 \\
			& 32 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{B40426} 0.00 & \cellcolor[HTML]{3F53C6} 538.12 & \cellcolor[HTML]{B40426} 37.00 & \cellcolor[HTML]{3B4CC0} 100.00 & \cellcolor[HTML]{E9D5CB} 36.88 & \cellcolor[HTML]{B40426} 1048.70 \\
		\end{tabular}
	}
	\caption{Depicting the balance between performance and safety with regards to STL specification complexity for the DoubleIntegrator Environment at various scales.}
	\label{tab:double-safety-performance}
\end{table*}
